The WiLI benchmark dataset for written language identification

This paper describes the WiLI-2018 benchmark dataset for monolingual written natural language identification. WiLI-2018 is a publicly available, free of charge dataset of short text extracts from Wikipedia. It contains 1000 paragraphs of 235 languages, totaling in 23500 paragraphs. WiLI is a classification dataset: Given an unknown paragraph written in one dominant language, it has to be decided which language it is.

==> Makefile <==
DOKUMENT = main

make:
	pdflatex $(DOKUMENT).tex -output-format=pdf # Referenzen erstellen
	bibtex $(DOKUMENT)
	pdflatex $(DOKUMENT).tex -output-format=pdf # Referenzen einbinden
	pdflatex $(DOKUMENT).tex -output-format=pdf # Referenzen einbinden
	make clean

ebook:
	latexml --dest=$(DOKUMENT).xml $(DOKUMENT).tex
	latexmlpost -dest=$(DOKUMENT).html $(DOKUMENT).xml
	ebook-convert $(DOKUMENT).html $(DOKUMENT).epub --language de --no-default-epub-cover

check:
	aspell -c -t content.tex

arxiv:
	zip -r upload.zip . -x \*.git\* -x MAKEFILE -x *.zip -x *.pdf

clean:
	rm -rf $(TARGET) *.class *.html *.aux *.out *.thm *.idx *.toc *.ilg *.glg *.glo *.gls *.ist *.xdy *.fdb_latexmk *.bak *.blg *.glsdefs *.acn *.acr *.alg *.nls *.nlo *.bak *.pyg *.lot *.lof *.xmpdata *.xmpi
	rm -rf _minted-booka4
	rm -rf *.log  # Analyze this for errors
	#rm -rf *.bbl *.ind  # Needed for arxiv
